Scalable Fault-Tolerant MapReduce

Supercomputers getting ever larger and energy-efficient is at odds with the reliability of the used hardware. Thus, the time intervals between component failures are decreasing. Contrarily, the latencies for individual operations of coarse-grained big-data tools grow with the number of processors. To overcome the resulting scalability limit, we need to go beyond the current practice of interoperation checkpointing. We give first results on how to achieve this for the popular MapReduce framework where huge multisets are processed by user-defined mapping and reducing functions. We observe that the full state of a MapReduce algorithm is described by its network communication. We present a low-overhead technique with no additional work during fault-free execution and the negligible expected relative communication overhead of $1/(p-1)$ on $p$ PEs. Recovery takes approximately the time of processing $1/p$ of the data on the surviving PEs. We achieve this by backing up self-messages and locally storing all messages sent through the network on the sending and receiving PEs until the next round of global communication. A prototypical implementation already indicates low overhead $<4\,\%$ during fault-free execution.

==> setup/pgfplots.tex <==

\usepackage{pgfplots}
\pgfplotsset{compat=1.16}

\usepgfplotslibrary{groupplots}
\usetikzlibrary{shapes.geometric,shapes.arrows,patterns,math}

\ifcmyk
\makeatletter
\def\pgfsys@setpatternuncolored#1#2#3#4#5{%
  \pgfsysprotocol@literal{/pgfpcmyk cs #2 #3 #4 #5 /pgfpat#1\space scn}%
}
\def\pgf@sys@pgf@resource@list@colorspaces{} %
\pgfutil@addpdfresource@colorspaces{ /pgfpcmyk [/Pattern /DeviceCMYK] }

\def\pgf@set@fillpattern#1#2{%
  \pgfutil@ifundefined{pgf@pattern@name@#1}{%
    \pgferror{Undefined pattern `#1'}}
  {%
    \csname pgf@pattern@instantiate@#1\endcsname%
    \expandafter\global\expandafter\let\csname pgf@pattern@instantiate@#1\endcsname=\relax%
    \pgf@ifpatternisinherentlycolored{#1}{%
      \pgfsys@setpatterncolored{\csname pgf@pattern@name@#1\endcsname}%
    }{%
      \pgfutil@colorlet{pgf@tempcolor}{#2}%
      \pgfutil@ifundefined{applycolormixins}{}{\applycolormixins{pgf@tempcolor}}%
      \pgfutil@extractcolorspec{pgf@tempcolor}{\pgf@tempcolor}%
      \expandafter\pgfutil@convertcolorspec\pgf@tempcolor{cmyk}{\pgf@cmykcolor}%
      \expandafter\pgf@set@fill@patternuncolored\pgf@cmykcolor\relax{#1}%
    }%
  }%
}
\def\pgf@set@fill@patternuncolored#1,#2,#3,#4\relax#5{%
  \pgfsys@setpatternuncolored{\csname pgf@pattern@name@#5\endcsname}{#1}{#2}{#3}{#4}%
}
\makeatother
\fi %

\definecolor{plotcolor0}{RGB}{255,0,0}
\definecolor{plotcolor1}{RGB}{0,0,255}
\definecolor{plotcolor2}{RGB}{64,170,0}
\definecolor{plotcolor3}{RGB}{170,0,255}
\definecolor{plotcolor4}{RGB}{0,170,255}
\definecolor{plotcolor5}{RGB}{164,164,0}
\definecolor{plotcolor6}{RGB}{128,128,128}
\definecolor{plotcolor7}{RGB}{0,0,0}
\definecolor{plotcolor8}{RGB}{0,110,165}
\definecolor{plotcolor9}{RGB}{128,64,0}

\pgfplotscreateplotcyclelist{mycolor}{%
  plotcolor0, every mark/.append style={solid,scale=0.8}, mark=x \\%
  plotcolor1, every mark/.append style={solid,scale=0.6}, mark=o \\%
  plotcolor2, every mark/.append style={solid,scale=0.8}, mark=diamond \\%
  plotcolor3, every mark/.append style={solid,scale=0.8}, mark=triangle \\%
  plotcolor4, every mark/.append style={solid,scale=0.8,rotate=180}, mark=triangle \\%
  plotcolor5, every mark/.append style={solid,scale=0.65}, mark=square \\%
  plotcolor6, every mark/.append style={solid,scale=0.8}, mark=star \\%
  plotcolor7, every mark/.append style={solid,scale=0.8}, mark=+ \\%
  plotcolor8, every mark/.append style={solid,scale=0.8}, mark=pentagon \\%
  plotcolor9, every mark/.append style={solid,scale=0.9}, mark=Mercedes star flipped \\%
  plotcolor0, every mark/.append style={solid,scale=0.8}, mark=x, dashed \\%
  plotcolor1, every mark/.append style={solid,scale=0.6}, mark=o, dashed \\%
  plotcolor2, every mark/.append style={solid,scale=0.8}, mark=diamond, dashed \\%
  plotcolor3, every mark/.append style={solid,scale=0.8}, mark=triangle, dashed \\%
  plotcolor4, every mark/.append style={solid,scale=0.8,rotate=180}, mark=triangle, dashed \\%
  plotcolor5, every mark/.append style={solid,scale=0.65}, mark=square, dashed \\%
  plotcolor6, every mark/.append style={solid,scale=0.8}, mark=star, dashed \\%
  plotcolor7, every mark/.append style={solid,scale=0.8}, mark=+, dashed \\%
  plotcolor8, every mark/.append style={solid,scale=0.8}, mark=pentagon, dashed \\%
  plotcolor9, every mark/.append style={solid,scale=0.9}, mark=Mercedes star flipped, dashed \\%
  plotcolor0, every mark/.append style={solid,scale=0.8}, mark=x, densely dotted \\%
  plotcolor1, every mark/.append style={solid,scale=0.6}, mark=o, densely dotted \\%
  plotcolor2, every mark/.append style={solid,scale=0.8}, mark=diamond, densely dotted \\%
  plotcolor3, every mark/.append style={solid,scale=0.8}, mark=triangle, densely dotted \\%
  plotcolor4, every mark/.append style={solid,scale=0.8,rotate=180}, mark=triangle, densely dotted \\%
  plotcolor5, every mark/.append style={solid,scale=0.65}, mark=square, densely dotted \\%
  plotcolor6, every mark/.append style={solid,scale=0.8}, mark=star, densely dotted \\%
  plotcolor7, every mark/.append style={solid,scale=0.8}, mark=+, densely dotted \\%
  plotcolor8, every mark/.append style={solid,scale=0.8}, mark=pentagon, densely dotted \\%
  plotcolor9, every mark/.append style={solid,scale=0.9}, mark=Mercedes star flipped, densely dotted \\%
}

\pgfplotscreateplotcyclelist{reservoir}{%
  plotcolor0, every mark/.append style={solid,fill opacity=0.6,scale=1}, mark=diamond* \\%
  plotcolor1, every mark/.append style={solid,fill opacity=0.6,scale=0.8}, mark=square* \\%
  plotcolor2, every mark/.append style={solid,fill opacity=0.6,scale=1}, mark=* \\%
  plotcolor0, every mark/.append style={solid,fill opacity=0.2,scale=1}, mark=diamond*, dashed \\%
  plotcolor1, every mark/.append style={solid,fill opacity=0.2,scale=0.8}, mark=square*, dashed \\%
  plotcolor2, every mark/.append style={solid,fill opacity=0.2,scale=1}, mark=*, dashed \\%
  plotcolor0, every mark/.append style={solid,scale=1}, mark=diamond, densely dotted \\%
  plotcolor1, every mark/.append style={solid,scale=0.8}, mark=square, densely dotted \\%
  plotcolor2, every mark/.append style={solid,scale=1}, mark=o, densely dotted \\%
}


\definecolor{mlblue}{RGB}{114,147,203}
\definecolor{mlbrown}{RGB}{225,151,76}
\definecolor{mlgreen}{RGB}{132,186,91}
\definecolor{mlred}{RGB}{211,94,96}
\definecolor{mlgray}{RGB}{128,133,133}
\definecolor{mlpurple}{RGB}{144,103,167}
\definecolor{mlox}{RGB}{171,104,87}
\definecolor{mlmoss}{RGB}{204,194,16}

\definecolor{mdblue}{RGB}{57,106,177}
\definecolor{mdbrown}{RGB}{218,124,48}
\definecolor{mdgreen}{RGB}{62,150,81}
\definecolor{mdred}{RGB}{204,37,41}
\definecolor{mdgray}{RGB}{83,81,84}
\definecolor{mdpurple}{RGB}{107,76,154}
\definecolor{mdox}{RGB}{146,36,40}
\definecolor{mdmoss}{RGB}{148,139,61}

\pgfplotscreateplotcyclelist{wrscons}{%
  {mdblue,every mark/.append style={fill=mlblue},mark=*},%
  {mdred,every mark/.append style={fill=mlred},mark=*},%
  {mdbrown,every mark/.append style={fill=mlbrown},mark=square*},%
  {mdgray,every mark/.append style={fill=mlgray},mark=diamond*},%
  {mdpurple,every mark/.append style={fill=mlpurple},mark=diamond*}%
}
\pgfplotscreateplotcyclelist{wrsquery}{%
  {mdred,every mark/.append style={fill=mlred},mark=*},%
  {mdbrown,every mark/.append style={fill=mlbrown},mark=square*},%
  {mdgreen,every mark/.append style={fill=mlgreen},mark=square*},%
  {mdgray,every mark/.append style={fill=mlgray},mark=diamond*}%
}


\makeatletter
\pgfdeclarepatternformonly[\GridSize]{MyFill}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{\GridSize}{\GridSize}}{\pgfqpoint{\GridSize}{\GridSize}}%
{
  \pgfsetcolor{\tikz@pattern@color}
  \pgfsetlinewidth{0.3pt}
  \pgfpathmoveto{\pgfqpoint{0pt}{0pt}}
  \pgfpathlineto{\pgfqpoint{\GridSize}{\GridSize}}
  \pgfusepath{stroke}
}
\makeatother
\newdimen\GridSize
\tikzset{
    GridSize/.code={\GridSize=#1},
    GridSize=4.25pt
}


\makeatletter
\pgfplotsset{
    groupplot xlabel/.initial={},
    every groupplot x label/.style={
        at={($({\pgfplots@group@name\space c1r\pgfplots@group@rows.west}|-{\pgfplots@group@name\space c1r\pgfplots@group@rows.outer south})!0.5!({\pgfplots@group@name\space c\pgfplots@group@columns r\pgfplots@group@rows.east}|-{\pgfplots@group@name\space c\pgfplots@group@columns r\pgfplots@group@rows.outer south})$)},
        anchor=north,
    },
    groupplot ylabel/.initial={},
    every groupplot y label/.style={
            rotate=90,
        at={($({\pgfplots@group@name\space c1r1.north}-|{\pgfplots@group@name\space c1r1.outer
west})!0.5!({\pgfplots@group@name\space c1r\pgfplots@group@rows.south}-|{\pgfplots@group@name\space c1r\pgfplots@group@rows.outer west})$)},
        anchor=south
    },
    execute at end groupplot/.code={%
      \node [/pgfplots/every groupplot x label]
{\pgfkeysvalueof{/pgfplots/groupplot xlabel}};
      \node [/pgfplots/every groupplot y label]
{\pgfkeysvalueof{/pgfplots/groupplot ylabel}};
    }
}
\def\endpgfplots@environment@groupplot{%
    \endpgfplots@environment@opt%
    \pgfkeys{/pgfplots/execute at end groupplot}%
    \endgroup%
}
\makeatother


\newenvironment{customlegend}[1][]{%
  \begingroup\csname pgfplots@init@cleared@structures\endcsname\pgfplotsset{#1}%
}{\csname pgfplots@createlegend\endcsname\endgroup}%
\def\addlegendimage{\csname pgfplots@addlegendimage\endcsname}


\makeatletter
\newif\ifhidelinks@hidelinks
\newcommand{\hidelinks}{%
  \hidelinks@hidelinkstrue
  \let\hidelinks@ifHy@colorlinks@status\ifHy@colorlinks
  \let\hidelinks@ifHy@ocgcolorlinks@status\ifHy@ocgcolorlinks
  \let\hidelinks@ifHy@frenchlinks@status\ifHy@frenchlinks
  \let\hidelinks@Hy@colorlink\Hy@colorlink
  \let\hidelinks@Hy@endcolorlink\Hy@endcolorlink
  \let\hidelinks@@pdfborder\@pdfborder
  \let\hidelinks@@pdfborderstyle\@pdfborderstyle
  \hypersetup{hidelinks}%
}
\newcommand{\restorelinks}{%
  \ifhidelinks@hidelinks
    \hidelinks@hidelinksfalse
    \let\ifHy@colorlinks\hidelinks@ifHy@colorlinks@status
    \let\ifHy@ocgcolorlinks\hidelinks@ifHy@ocgcolorlinks@status
    \let\ifHy@frenchlinks\hidelinks@ifHy@frenchlinks@status
    \let\Hy@colorlink\hidelinks@Hy@colorlink
    \let\Hy@endcolorlink\hidelinks@Hy@endcolorlink
    \let\@pdfborder\hidelinks@@pdfborder
    \let\@pdfborderstyle\hidelinks@@pdfborderstyle
  \fi
}
\makeatother


\pgfplotsset{
    box plot/.style={
        /pgfplots/.cd,
        black,
        only marks,
        mark=-,
        mark size=\pgfkeysvalueof{/pgfplots/box plot width},
        /pgfplots/error bars/y dir=plus,
        /pgfplots/error bars/y explicit,
        /pgfplots/table/x index=\pgfkeysvalueof{/pgfplots/box plot x index},
    },
    box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw  ##1 -- ++(\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##2 -- ++(-\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot box top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
        },
        /pgfplots/box plot
    },
    box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker top index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box top index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker top index}}
        },
        /pgfplots/box plot
    },
    box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=\pgfkeysvalueof{/pgfplots/box plot whisker bottom index},
        y error expr={
            \thisrowno{\pgfkeysvalueof{/pgfplots/box plot box bottom index}}
            - \thisrowno{\pgfkeysvalueof{/pgfplots/box plot whisker bottom index}}
        },
        /pgfplots/box plot
    },
    box plot median/.style={
        /pgfplots/box plot,
        /pgfplots/table/y index=\pgfkeysvalueof{/pgfplots/box plot median index}
    },
    box plot width/.initial=1em,
    box plot x index/.initial=0,
    box plot median index/.initial=3,
    box plot box top index/.initial=4,
    box plot box bottom index/.initial=2,
    box plot whisker top index/.initial=5,
    box plot whisker bottom index/.initial=1,
}

\newcommand{\boxplot}[2][]{
    \addplot [box plot median,#1] table {#2};
    \addplot [forget plot, box plot box,#1] table {#2};
    \addplot [forget plot, box plot top whisker,#1] table {#2};
    \addplot [forget plot, box plot bottom whisker,#1] table {#2};
}

